Icebreaker: Element-wise Active Information Acquisition with Bayesian Deep Latent Gaussian Model

In this paper we introduce the ice-start problem, i.e., the challenge of deploying machine learning models when only little or no training data is initially available, and acquiring each feature element of data is associated with costs. This setting is representative for the real-world machine learning applications. For instance, in the health-care domain, when training an AI system for predicting patient metrics from lab tests, obtaining every single measurement comes with a high cost. Active learning, where only the label is associated with a cost does not apply to such problem, because performing all possible lab tests to acquire a new training datum would be costly, as well as unnecessary due to redundancy. We propose Icebreaker, a principled framework to approach the ice-start problem. Icebreaker uses a full Bayesian Deep Latent Gaussian Model (BELGAM) with a novel inference method. Our proposed method combines recent advances in amortized inference and stochastic gradient MCMC to enable fast and accurate posterior inference. By utilizing BELGAM's ability to fully quantify model uncertainty, we also propose two information acquisition functions for imputation and active prediction problems. We demonstrate that BELGAM performs significantly better than the previous VAE (Variational autoencoder) based models, when the data set size is small, using both machine learning benchmarks and real-world recommender systems and health-care applications. Moreover, based on BELGAM, Icebreaker further improves the performance and demonstrate the ability to use minimum amount of the training data to obtain the highest test time performance.

==> coldstart.tex <==

% \begin{figure}[t]
% \centering
% \begin{minipage}[c]{0.4\textwidth}
% \includegraphics[scale=0.2]{tikz/Active_training_diagram.pdf}
% \caption{The flow diagram of active training phase at time $t-1$.}
% \label{fig:active training t-1}
% \end{minipage}
% \hfill
% \begin{minipage}[c]{0.4\textwidth}
% \includegraphics[scale=0.23]{tikz/PVAE_Encoer.pdf}
% \caption{The illustration of P-VAE inference network structure.}
% \label{fig:P-VAE inference net}
% \end{minipage}
% \end{figure}

\begin{figure}
\subfloat[]{\includegraphics[scale=0.2]{tikz/Active_training_diagram.pdf}\label{fig:active training t-1}}\hfill
\subfloat[]{ \begin{minipage}{0.4\textwidth}\vspace{-2cm}\includegraphics[scale=0.23]{tikz/PVAE_Encoer.pdf}\label{fig:P-VAE inference net}\end{minipage}}
\caption{(\textbf{Left}) The flow diagram of active training phase at time $t-1$. (\textbf{Right}) The illustration of P-VAE inference network structure. \CZ{The font of (a) has not fixed yet.}}
\end{figure}
Assume at each acquisition step we have training data $\mathcal{D}_{train}$, a pool data set $\mathcal{D}_{pool}$ \wg{that contain the data we could query} and $\mathcal{D}_{train}\cup\mathcal{D}_{pool}= \bm{X}\in \mathbb{R}^{N\times D}$, \cmmnt{\cz{$\mathcal{D}_{train}$ indicates the data that we have collected for training.}} in the ice-start scenario, $\mathcal{D}_{train} = \emptyset$. $\mathcal{D}_{pool}$ is the pool data that we can possibly acquire. At each step of the training-time acquisition, we actively select data points $x_{i,d}\in\mathcal{D}_{pool}$ to acquire, thereby moving them into $\mathcal{D}_{train}$ and updating the model with the newly formed $\mathcal{D}_{train}$. Figure \ref{fig:active training t-1} shows the flow diagram of this procedure. During the process, at any step, there is an observed data set $\bm{X}_O$ and unobserved set $\bm{X}_U$ with $|O|$ and $|U|$ number of rows respectively. For each (partially observed) data instance $\bm{x}_i\in \bm{X}_O$, we have the observed index set $O_i$ containing index of observed features for row $i$. If the data set has a clear target variable, we denote the target as $\bm{Y}$. In this case, each $\bm{x}_i\in\bm{X}_O$ has a corresponding target $\bm{y}_i$.


% \cz{The Icebreaker is desired to be able to select points that are 
% informative for model training. Thus, a model which 'knows what is unknown' and an objective function ,which }\wg{trades off between exploration of new features and exploitation of informative ones, are needed}
% trades off the model uncertainty with the performance of test tasks are needed.}
In this project, we consider two test tasks with test set $\mathcal{D}_{test}$: (i) \textit{Imputation}: We have $\bm{X}^*_O\cup\bm{X}^*_U=\mathcal{D}_{test}$ and an evaluation metric $f(\cdot)$, e.g., negative log likelihood. The task is to evaluate the performance $f(\bm{X}^*_U)$ given $\bm{X}^*_O$ and, (ii) \textit{Active Prediction}: We have an additional target $\bm{Y}^*$. At each test time query, a single feature $x^*_{id}\in \bm{X}^*_U$ for each row $i$ is moved into $\bm{X}^*_O$. The goal is to achieve better target prediction \wg{$f(\bm{Y}^*,\tilde{\bm{Y}}^*)$ with minimal data queries, where $\tilde{\bm{Y}}^*$ are the predicted targets conditioned on $\bm{X}^*_O$}.\CZ{The previous sentence needs rewriting f is not clear} We include the detailed procedures (both training and test) in the appendix \ref{subsec: acquisition procedure}. 
% \wg{For active prediction in medical domain, the $\bm{X}_O$, $\bm{X}_U$ may represent the measurements that has been taken and remaining possible tests respectively. Target $\bm{Y}$ is the diagnosis of the patients.  }



==> tikz_PNP.tex <==
%auto-ignore
\pgfdeclarelayer{background}
\pgfdeclarelayer{foreground}
\pgfsetlayers{background,main,foreground}

\definecolor{babyblue}{rgb}{0.54, 0.81, 0.94}
\definecolor{bisque}{rgb}{1.0, 0.89, 0.77}
\definecolor{bittersweet}{rgb}{1.0, 0.44, 0.37}

\begin{tikzpicture}


\tikzstyle{surround} = [thick,draw=black,rounded corners=1mm]
\tikzstyle{scalarnode} = [circle, draw, fill=white!11,  
    text width=1.2em, text badly centered, inner sep=2.5pt]
\tikzstyle{scalarnodenoline} = [  fill=white!11, 
    text width=1.2em, text badly centered, inner sep=2.5pt]
\tikzstyle{arrowline} = [draw,color=black, -latex]
\tikzstyle{dashedarrowcurve} = [draw,color=black, dashed, out=100,in=250, -latex]
\tikzstyle{dashedarrowline} = [draw,color=black, dashed,  -latex]

\node [] at (0.2+8,0.5) (ip2) {\small $(|O|, M)$};

%%e%%
\node (rect) at (0+8,0) [draw,thick, fill=babyblue, minimum width=1.5cm, minimum height=0.5cm] (e1){$e_1$};

\node [] at (0+8,-1) {$...$};

\node (rect) at (0+8,-1.5) [draw,thick,fill=babyblue,minimum width=1.5cm, minimum height=0.5cm] (e4) {$e_{|O|}$};

%%x%%
\node (rect) at (0.7+8,-0.7) [draw,thick, fill=bisque, minimum width=0.75cm, minimum height=0.5cm] (x1){$x_1$};

\node (rect) at (0.7+8,-2.2) [draw,thick,fill=bisque,minimum width=0.75cm, minimum height=0.5cm] (x4){$x_{|O|}$};

%%*%%
\node [circle] at (1.2+8+0.2,-0.3) [draw,thick, fill=black!50, minimum width=0.3cm, minimum height=0.3cm,inner sep=0pt] (m1){$\times$};

\node [circle] at (1.2+8+0.2,-1.8) [draw,thick,fill=black!50,minimum width=0.3cm, minimum height=0.3cm, inner sep=0pt] (m4){$\times$};


\node (rect)  at (2.5+8+0.2,-0.5) [draw, rounded rectangle,thick,inner sep=0pt, fill=blue!50, minimum width=1.5cm, minimum height=0.35cm] (h1) { \small $h$};


\node [scalarnodenoline] at (2.25+8+0.2,-1) (s1) {shared};

\node (rect) at (2.5+8+0.2,-1.6) [draw, rounded rectangle,thick,inner sep=0pt,fill=blue!50,minimum width=1.5cm, minimum height=0.35cm] (h4){  \small$h$};

\node (circle) at (4+8,-1) [draw,thick, fill=black!50, minimum width=0.4cm, minimum height=0.4cm] (g2) {g};
\path [arrowline]  (x1) to (m1);
\path [arrowline]  (x4) to (m4);
\path [arrowline]  (e1) to (m1);
\path [arrowline]  (e4) to (m4);
\path [arrowline]  (m1) to (h1);
\path [arrowline]  (m4) to (h4);
\path [arrowline]  (h1) to (g2);
\path [arrowline]  (h4) to (g2);


\node [] at (5+8,-0.5) (ip) {\small $(1,K)$};

\node (rect) at ( 5+8,-1) [draw,thick, fill=bittersweet, minimum width=0.8cm, minimum height=0.4cm] (c2) {$ c$};

\path [arrowline]  (g2) to (c2);


\node (rect) at ( 6+8,-1) [draw,thick, rotate=90, fill=black!50, minimum width=0.4cm, minimum height=0.4cm] (conc2) {ENCODER};


\path [arrowline]  (c2) to (conc2);



\node (rect) at (2.4+8,-0.9) [draw,thick,dashed,minimum width=6.5cm, minimum height=3.3cm] {};


\end{tikzpicture}

